Resource Allocation in Quantum Networks for Distributed Quantum Computing

The evolution of quantum computing technologies has been advancing at a steady pace in the recent years, and the current trend suggests that it will become available at scale for commercial purposes in the near future. The acceleration can be boosted by pooling compute infrastructures to either parallelize algorithm execution or solve bigger instances that are not feasible on a single quantum computer, which requires an underlying Quantum Internet: the interconnection of quantum computers by quantum links and repeaters to exchange entangled quantum bits. However, Quantum Internet research so far has been focused on provisioning point-to-point flows only, which is suitable for (e.g.) quantum sensing and metrology, but not for distributed quantum computing. In this paper, after a primer on quantum computing and networking, we investigate the requirements and objectives of smart computing on distributed nodes from the perspective of quantum network provisioning. We then design a resource allocation strategy that is evaluated through a comprehensive simulation campaign, whose results highlight the key features and performance issues, and lead the way to further investigation in this direction.

==> motivation.tex <==
The initial graph is $\mathcal{G}'=(\mathcal{V},\mathcal{E})$.
Algorithm to allocate a new flow $f = (s, d, r, F_{\min}$):

\begin{myenumlist}
    \item select shortest path $p$ from $s$ to $d$, in terms of hops (this
    minimizes resource utilization and maximizes the fidelity of the
    end-to-end entangled pair); if there is no path, then admission control
    fails

    \item determine gross rate along the path selected as
    $r' = \frac{r}{q^{|p|-1}}$

    \item if $r' \geq \min_{i,j \in p} C_{ij}$ then go to next step;
    otherwise, remove the edge with minimum capacity from $\mathcal{G}'$
    and restart from 1.

    \item compute the fidelity $F'$ of the end-to-end entangled pair using
    \req{fidelity:perfect}: if $F' \geq F_{\min}$ then the flow can be
    admitted and all the capacities of the edges along $p$ must be updated
    for future requests by removing $r'$, otherwise admission control fails
\end{myenumlist}

Worst-case computational time complexity: $\mathcal{O}(K(E+V \log V))$, with
$K$ upper-bounded by $E$.

\myfigdoubleeps{num-edges}{max-degree}{graph-properties}{%
    Distribution of the number of edges (left) and vertices (right).}

\myfigdoubleeps{admission-cdf}{residual}{var-flows}{%
    Cumulative distribution of the admission rate (left) and residual capacity (right),
    as the number of flows increases,
    with $\mu = 100$ nodes and link capacity in $U[1,99]$.}

\myfigeps{admission}{%
    Average admission rate vs. number of flows.}

\myfigeps{admission-map}{%
    Average residual capacity / total capacity vs. admission rate,
    with $\mu = 100$ nodes and link capacity in $U[1,99]$.}

\myfigeps{dijkstra}{%
    Average number of Dijkstra's algorithm executions vs. number of flows.}

\myfigeps{admission-2}{%
    Average admission rate vs. link capacity.}

\myfigeps{admission-map-2}{%
    Residual capacity vs. admission rate,
    with $\mu = 100$ nodes and variable link capacities.}

\myfigeps{residual-2}{%
    Average residual capacity vs. link capacity.}

\myfigeps{residual-ratio}{%
    Average residual capacity / total capacity vs. link capacity.}

